Near-Infrared Mapping and Physical Properties of the Dwarf-Planet Ceres

We study the physical characteristics (shape, dimensions, spin axis direction, albedo maps, mineralogy) of the dwarf-planet Ceres based on high-angular resolution near-infrared observations. We analyze adaptive optics J/H/K imaging observations of Ceres performed at Keck II Observatory in September 2002 with an equivalent spatial resolution of ~50 km. The spectral behavior of the main geological features present on Ceres is compared with laboratory samples. Ceres' shape can be described by an oblate spheroid (a = b = 479.7 +/- 2.3 km, c = 444.4 +/- 2.1 km) with EQJ2000.0 spin vector coordinates RA = 288 +/- 5 deg. and DEC = +66 +/- 5 deg. Ceres sidereal period is measured to be 9.0741 +/- 0.0001 h. We image surface features with diameters in the 50-180 km range and an albedo contrast of ~6% with respect to the average Ceres albedo. The spectral behavior of the brightest regions on Ceres is consistent with phyllosilicates and carbonate compounds. Darker isolated regions could be related to the presence of frost.

==> sections/analysis.tex <==
\section{Data analysis\label{sec-analysis}}
%
%
%
  \subsection{Spin vector coordinates\label{subsec-pole-coordinates}}
%
    \indent Measuring the Spin Vector Coordinates (SVC) of Ceres has always been a difficult task. The small amplitude of its lightcurve ($\sim$0.04 mag) prevented its determination using classical lightcurve inversion techniques. Until recently, the solutions that were reported for the pole coordinates of Ceres were spanning a 90\degr range in the plane of  the sky (as shown by \citet{2002-AJ-123-Parker}). This situation changed dramatically with the use of direct imaging technique capable of resolving the disk of Ceres and image details on its surface (e.g. HST observations performed by \citet{2005-Nature-437-Thomas}, and this paper). The precise knowledge of the orientation of Ceres spin axis is mandatory to re-project the individual images into albedo maps of its surface. Although a first precise SVC for Ceres was reported by Thomas et al. (2005), we took the opportunity of analyzing our set of adaptive optics images to obtain an independent measurement of its value.\\
%
    \indent We performed a control-point method, which consist of following the apparent motion of a surface feature while the asteroid rotates. An albedo feature on the surface of Ceres draws a circle in a plane perpendicular to the rotation axis, while its apparent trajectory becomes an ellipse if the asteroid is seen under an aspect angle different from 90\degr. We marked the successive positions of two main features, A and B  (\textbf{Fig. \ref{fig-views-of-ceres}}), visible in 100 and 87 images resp., while the rotational phase of the asteroid  spanned a 93.9\degr and 87.7\degr range resp. All these measurements are shown together on a 3-D model of Ceres in \textbf{Fig. \ref{fig-CPM}}. The trajectory solution being directly linked to the orientation of the rotational axis, we were able to determine the north pole angle (\pn) and the sub-earth latitude (\be) at the time of the observations. In order to compare the solution with other studies we followed the IAU recommendations and calculated the SVC in the J2000.0 equatorial frame. We found \ra=287.6\degr and \dec=66.4\degr with an uncertainty of 5\degr on each value. This result is very close to the lastest result from HST \citep{2005-Nature-437-Thomas} but slightly different. The resolution element is almost the same in both studies but the pixel scale at Keck II is roughly twice as small as the ones from HST. The result is a Nyquist-sampling of the resolution element at Keck, whereas the ACS data coming from HST are Nyquist-sampled by combining 2$\times$2 resolution elements. Thus the spatial resolution within present study is higher than the one obtained with HST and we are so more confident about the present measurements. \\
%
    \indent This pole solution returns a small value for the obliquity of Ceres of about ......\degr, which was expected from the analysis of lightcurve data \citep{1983-Icarus-54-Tedesco} and thermal properties of Ceres regolith \citep{1990-Icarus-83-Spencer}. In contrast, a larger obliquity would lead to variations of the lightcurve of Ceres with the epoch, while such a phenomenon has never been reported. \\
%
%%%%%%------ FIGURE --- Begin --- Control Point Method ------%%%%%%
\begin{figure}
  \begin{center}
    \resizebox{0.6\hsize}{!}{\includegraphics{SpinVectorOrientation}}
    \caption{Apparent motion of two features during the Ceres rotation. Each color corresponds to a specific feature : the bright sits for the feature at 234\degr E, 23\degr N (here called A) and the dark for the one at 132\degr E, 20\degr N (B) (see \textbf{Fig. \ref{fig-views-of-ceres}} and \textbf{Fig. \ref{fig-jhk-maps}} to localize features). From the shape of the feature tracks we were able to determine the rotation axis orientation.}
   \label{fig-CPM}
  \end{center}
\end{figure}
%%%%%%------ FIGURE --- End --- Control Point Method ------%%%%%%
%
   \indent Giving its SVC, Ceres can only be observed over a Sub-Earth Point Latitude (SEP$_\varphi$) range of [-11\degr, 10\degr] (computed for the next 50 years). As a result, the high-latitude regions of Ceres are always observed tangentially from Earth, and we will have to wait for the arrival of the DAWN spacecraft to have a first clear view of its poles.
%
%
%
%
%
%
%
%
  \subsection{Rotational period}
%
%%%%%%------ TABLE --- Begin --- Rotation ------%%%%%%
\begin{table}
  \caption{Reference points used to compute the rotational period. We show here the Sub-Earth Point Longitude (SEP$_\lambda$) observed as well as the one corrected from the relative position of the Earth with respect to Ceres. That is the Sub-Earth Point Longitude that should be observed if the relative position of Ceres and the Earth were the same for the three observations.}
  \label{tab-JD-SEPlong}
  \centering
  \begin{tabular}{c c c}
    \hline\hline
    Julian Date & Obs. SEP$_\lambda$ (\degr E) & Corrected SEP$_\lambda$ (\degr E)\\
    \hline
    2452539.89402002   &   234.6 $\pm$ 2  &  234.6 $\pm$ 2  \\
    2452545.91545790   &   261.4 $\pm$ 2  &  262.7 $\pm$ 2  \\
    2453002.24128009   &   ~22.6 $\pm$ 5  &  283.9 $\pm$ 5  \\
    \hline
\end{tabular}
\end{table}
%%%%%%------ TABLE ---  End  --- Rotation ------%%%%%%
%
    \indent Until the very recent study by Chamberlain et al. [Icarus, in press], the latest Ceres rotational period measurement was the one performed by \citet{1983-Icarus-54-Tedesco} and the admitted value was of 9.075 $\pm$ 0.001 h. We took our study as an opportunity to refine this determination via a direct measurement. Indeed, as we spatially resolve the apparent disk of Ceres, we can have reference epochs at which we know the rotational phase (the apparition of the same albedo feature for instance). So the rotation rate must fit these references. Observations need to be time separated in order to observe the asteroid after many rotations, when the accumulation of a small error on the period is measurable. \\
%
    \indent So we use our two epochs (September 2002, the 22\second~and 28\nth) plus another one from the HST (December 2003, the 28\nth) which has been published by \citet{2005-Nature-437-Thomas, 2006-Icarus-182-Li, 2006-AdSpR-38-Parker} and released on the Small Body Nodes. We determined the rotational phase of these three epochs by checking the position of known features over the Ceres apparent disk. Then we used an ephemeris generator (here eproc from the IMCCE \citep{1998-IMCCE-Berthier}) to compute the rotational phase over the various reference points as it would be expected from the first reference point. To determine the Ceres sidereal period we needed to correct the observed Sub-Earth Point Longitude of the apparent motion of the Earth around Ceres (\textbf{Tab.} \ref{tab-JD-SEPlong}). Then we search for the rotation rate that match the phase of the three epochs. The \textbf{Tab. \ref{tab-RateVSecart}} show the rotation rate matching the reference epochs, given the uncertainty over the reference phases.
%
%
%
%
%
%%%%%%------ TABLE --- Begin --- Rotation Results ------%%%%%%
\begin{table}
  \caption{Determined rotation rates with their residual longitudinal differences at the second (t$_2$) and third (t$_3$) reference epochs. We only kept rotation rates whose predicted SEP$_\lambda$ were inside measurement uncertainties for the three epochs.}
  \label{tab-RateVSecart}
  \centering
  \begin{tabular}{c c c}
    \hline\hline
    Period $T$ (h) & $\Delta$ SEP$_\lambda$ (t$_2$) & $\Delta$ SEP$_\lambda$ (t$_3$) \\
    \hline
    9.07406     &     -1.05\degr  &  ..\degr \\
    \hline
\end{tabular}
\end{table}
%%%%%%------ TABLE ---  End  --- Rotation Results ------%%%%%%
%
%

    \indent All these periods are consistent with the \citet{1983-Icarus-54-Tedesco} value, \textbf{depends on results, here come the discussion}\\
%
    \indent With our determination of the SVC and the rotation rate, we defined a reference epoch that is: \textbf{here comes the values we put in MOVIS, RA--DEC in EQJ2000.0, Omega0, phi0--jd0------give the eproc solution number}
%
%
%
%
%
%
%
%
%
%
%
  \subsection{Dimensions\label{subsec-dimensions}}
%
%%%%%%------ FIGURE --- Begin --- Edge Detection ------%%%%%%
\begin{figure}
  \begin{center}
%%%--- Graphics from the EPS and Caption
    \resizebox{.49\hsize}{!}{\includegraphics{edge-good}}
    \resizebox{.49\hsize}{!}{\includegraphics{deviation}}
    \caption{Left: Edge shape (black) from limb detection and fitted ellipse (gray) in a typical case of the used images, with very faint deviation from the ellipse, well inside the resolution element size. To help reading, we put the resolution element in the bottom-left corner. Right: Measured deviations from the fitted ellipse as function of the sub-earth latitude. As the deviations are well inside the resolution element ($\sim$37 km in J-band) positive relief detection require repetitive detection of the same deviation after 180\degr or 360\degr rotation.}
    \label{fig-edge}
  \end{center}
\end{figure}
%%%%%%------ FIGURE --- End --- Edge Detection ------%%%%%%
%
    \indent As shown by Thomas et al. (2005), the shape of Ceres is the unique tool we have available to date to remotely investigate its internal structure. The $\sim$37km spatial resolution delivered by Keck-AO at the distance of Ceres  allows us to independently estimate the size and shape of the largest main-belt asteroids. We thus performed a wavelet analysis with a Laplacian of Gaussian (LoG) wavelet to detect the Ceres edges over 192 images. The LoG is very sensitive to variations of gradient, which permits to precisely detect the inflection point in the envelope of our Ceres deconvolved images. Any image presenting any Gibbs-kind oscillations or ringing effect suspicion was eliminated from this part of the analysis. We found Ceres to be rotationally symmetric as first reported from a preliminary analysis of the Keck-AO data by \citet{2003-DPS-Dumas}, and later confirmed by \citet{2005-Nature-437-Thomas}. From the analysis of our contour images we did not measure any deviation from our ellipsoidal model larger than $\sim$18 km (see \textbf{Fig. \ref{fig-edge}}). From this fit, we were able to determine the minor- and major- projected axes of Ceres and correct them respectively from the aspect and phase angle effects. We found that Ceres is well described by an oblate spheroid whose axis are $a=479.7 \pm 2.3$ km and $c=444.4 \pm 2.1$ km (1$\sigma$ dispersion for the fitted axis). These values are different by $\sim$10 km when compared to the measurements based on HST observations, which correspond to a two percent relative difference. Considering that the best size measurements of Ceres come from stellar occultation, \citet{1987-Icarus-72-Millis} reported an independent measurement of the  semi-major axis of Ceres of $479.6 \pm 2.4$ km. The agreement between our values and the determination of the semi-major axis of Ceres made from stellar occultation is remarkable. However, our minor-axis value differ from theirs. Whereas they assumed a zero-obliquity and then underestimate the Sub-Earth Point Latitude (SEP$_\varphi$) at time of the occultation, the computation with our SVC solution give a SEP$_\varphi$ of -0.3\degr N. This implies a very small correction of the minor-axis from its projected value onto the plane of the sky. So we find a corrected polar radius from stellar occultation of $453.4 \pm 4.5$ km. As a result, our AO measurements agree within the uncertainties of the values reported from stellar occultation data.\\
%
    \indent The mean radius for Ceres is estimated to be $R=467.3 \pm 2.2$ km. Adopting a mass of $9.43 \pm 0.05 \times 10^{20}$ kg (corresponding to an average of lastest measurements \citep{1998-AA-334-Viateau,2000-AA-360-Michalak} done by \citet{2005-JGR-110-McCord}), we find a mean density of $\rho=2206 \pm 43$ kg.m$^{-3}$. This value is small for a rocky body and can be better compared  with the density of the outer Galilean satellites Ganymede and Callisto, than that of the inner Main Belt asteroids. One can now inverse the relation between $a$, $c$ and \Jdeux~\citep[given by][]{2005-JGR-110-McCord} as following
%
$$
      \Jdeux = \left[1 - \frac{c}{a} - \frac{2 \pi^{2} R^{3} }{T^{2} G M} \right]\left[ \frac{c}{2a} + \left( \frac{a}{c} \right)^{2} \right]^{-1}
$$
%
    \noindent and find $\Jdeux=26.7 \times 10^{-3} \pm 1.9 \times 10^{-5}$. By comparison, Thomas et al. (2005) $a$ and $c$ measurements lead to $\Jdeux=21.7 \times 10^{-3} \pm 8.5 \times 10^{-5}$. If we refer to \cite{2005-JGR-110-McCord}, these two independent estimates  of \Jdeux~correspond to internal models \# 2 and \# 3 for Ceres, that is to a differentiated Ceres with a silicate-rich region in its center. Whereas the \Jdeux~values are not the same according to the two high-angular resolution studies, they still converge towards a differentiated body as a model for Ceres. Nonetheless, the \Jdeux~value is highly dependant on the $a$ over $c$ ratio, so we may not take \Jdeux~information as final conclusion due to the spatial resolution reachable from earth. In the end, gravity field measurement from orbit will provide better understanding of mass repartition and internal structure.\\
%
    \indent We also measured the deviation of our contours from the fitted ellipse and report that no deviation greater than 18 km has been observed. This means that no topographic features larger than 18 km have been detected on Ceres with this study. This brings the question of the theoretical maximal height of a ``\textsl{mountain}'' on Ceres. We mean by ``\textsl{mountain}'' any topographic feature (true mountain, volcano or surrounding walls from impact crater...) and we modeled it by a cone of radius $b$ and height $h$. Following the \citet{1981-AA-2-Scheuer} work, we supposed that the height was limited by the material resistance and the ``\textsl{mountain}'' slope (if the slope is too high, a rock placed atop will slide/roll down). This gave a theoretical maximal height of
$$
      h = \sqrt{\frac{Y}{\rho_s g}} \sqrt{b}
$$

    \noindent where $Y$ is the shear strength (typically $1.5\times 10^{6}$ Pa for granite which is a good reference for silicate materials), $g$ is the surface gravity (0.288 m.s$^{-2}$) and $\rho_s$ is the density of the surface layer (corresponding to lithosphere on Earth): we used $\rho_s = 2206$ kg.m$^{-3}$ for an homogeneous Ceres and $\rho_s \simeq 1700$ kg.m$^{-3}$ for a differentiated Ceres, with a core density of $3440$ kg.m$^{-3}$ (model \# 2). The result is shown in \textbf{Fig. \ref{fig-Mountain}} for a mountain base radius spanning from 0 km up to 100 km (which is the range of observed structures on Ceres surface). We see that the highest feature we could expect on Ceres is about 15 km high for an homogeneous Ceres and a little higher ($\sim$18 km) if Ceres is differentiated. This result is of the same order of the results from the study by \citet{1973-Icarus-18-Johnson} based on assumptions made on material strengths and creep deformation for small bodies. As a result, it is expected that we do not detect any features departing from an ellipsoid fit of Ceres shape by more than nearly 18 km and the observed deviations may be reliefs on the surface. But as the variations are inside the resolution element, we need to detect them repeatedly (after 180\degr or 360\degr rotation for instance) to be sure that they are not high-frequency noise coming from the sampling of the data.

%
%
%
%
%%%%%%------ FIGURE --- Begin --- How high can be a Mountain ? ------%%%%%%
\begin{figure}
  \begin{center}
    \resizebox{\hsize}{!}{\includegraphics{mountain}}
    \caption{Theoretical mountain maximum height as function of the basis size. The line sits for $\rho_s=2206$ kg.m$^{-3}$ (homogeneous case) and the dots for $\rho_s \simeq 1700$ kg.m$^{-3}$ (differentiated case). The largest feature (A, see \textbf{Fig. \ref{fig-views-of-ceres}}) sustains a diameter of about 180 km, our chosen maximal basis. We see that any relief would be lower than approximately 18 km for the present albedo feature scale.}
    \label{fig-Mountain}
  \end{center}
\end{figure}
%%%%%%------ FIGURE --- End --- How high can be a Mountain ? ------%%%%%%
%
%
%
%
%
%
%
%
%
%
%
  \subsection{Near infrared maps\label{subsec-NIRmaps}}
%
    \indent The landmarks present on the surface of a planetary body (albedo marks, geological features) are best represented when projected onto a map. Their location and physical extent can directly be assessed and comparison with independent studies of the same object are easier to make.
%
%
%
%
%%%%%%------ Cylindrical Equidistant Projection Choice ------%%%%%%
    \paragraph*{Projection:} As any projection of a sphere or an ellipsoid onto a plane introduces deformations \citep{SurfaceMapping}, we attempted to minimize their effects by choosing the cylindrical equidistant projection. This projection consists to map the surface of the object onto a cylinder tangent to its equator while conserving the distances along the meridians. It minimizes the deformations in the equatorial region, which was the area of main interest: the low Sub-Earth Point Latitude ($\sim$12\degr N) at the time of observation offered an almost direct view of the equatorial region while the deformations were extremely strong at higher planetocentric latitudes. Other observational conditions (e.g. a greater Sub-Earth Point Latitude) would have led to another choice of projection \citep[see][for further reading]{SurfaceMapping}.
%
%
%
%
%
%%%%%%------ Definition of a ROI ------%%%%%%
    \paragraph*{Region of interest :} Although all images used to produce the maps were carefully cleaned (including from correlated noise) before deconvolution, some of them still presented artifacts after their optimal resolution had been restored, particularly near discontinuities such as the limb and terminator. Although \mistral~was designed to optimally process objects with sharp edges by preventing Gibbs-kind oscillations at the boundaries, it appeared difficult in certain cases to restore the edge profile while preserving the surface details, which was our main objective. At the same time, the resolution per pixel is higher at the center of the apparent disk than on its border since each pixel corresponds to a smaller physical area (this effect is easily understandable by looking the regularly spacing grid in the \textbf{Fig. \ref{fig-CPM}}). Thus, averaging elements of images coming from pixels near the border of the object would degrade the optimal resolution provided by the pixels from the center. Based on these considerations, we produce albedo maps of Ceres using only the pixels located within an ellipsoidal Region Of Interest (ROI) centered on the image, and whose semi-axes were equal to 80\% of the corresponding projected semi-axes on Ceres. The ROI corresponds to 64\% of the projected surface for each image (see \textbf{Fig. \ref{fig-3DvsIM}} to have a ROI representation over Ceres view).
%
%
%
%
%%%%%%------ Luminuous gradient correction ------%%%%%%
    \paragraph*{Phase angle correction: }  All our images presented a high gradient of luminosity across the disk of Ceres, which was introduced by a non-zero phase angle at the time of observation. Since any area of the map was obtained by averaging images corresponding to different rotational phases, hence affected at different degrees by the gradient of luminosity, we had to correct the individual images from this effect. We tried several diffusion law such as the Lambert, Lommel-Seelinger, Minnaert and Hakpe (including single-scattering and multiple-scattering effects) laws \citep[see][]{hapke-theory}. We also attempted to model the surface by a simple plane. Then we compared the root mean square of the Ceres surface minus the model. Among the usual laws, the Hapke one was found to best fit the Ceres surface, but its rms was still twice larger that the residual obtained from the plane model. We therefore adopted a plane model to correct all our images from the luminosity gradient before their projection into maps. 
%
%
%
%
%%%%%%------ From (x,y) frame to (lambda,phi) one ------%%%%%%
    \paragraph*{Projection :} The main difficulty encountered during the conversion from the original image to its planetocentric referential longitude ($\lambda$) and latitude ($\varphi$), as recommended by the IAU, \citep{2005-CeMDA-91-Seidelmann}), is to find the precise location of the center of the referential. As the distribution of the gravity field is unknown for Ceres, we made the assumption that its center of mass coincides with the geometrical center of our images. The determination of the referential center could be done from our knowledge of the asteroid dimensions (see \ref{subsec-dimensions}) and its orientation in space (SVC, see \ref{subsec-pole-coordinates}). This lastest information is given by three quantities : the north pole angle (\pn), the Sub-Earth Point Latitude (SEP$_\varphi$) and the Sub-Earth Point Longitude (SEP$_\lambda$), which can be computed after an arbitrary reference meridian is defined. We used the MOVIS ephemeris generator \citep{1998-IMCCE-Berthier} to obtain these quantities at the time of each observation. \\
%
%
%
%
%%%%%%------ Worldwide map from individual ones ------%%%%%%
    \paragraph*{Mosaicking :} Before combining all the individual projections onto maps of Ceres, we needed to correct each projection from its corresponding atmospheric extinction. We did not make any particular assumption about the correspondence between a particular view and the phase of Ceres lightcurve. We adjust each image flux level to that of its closer neighbors. Doing so, we preserved the flux variation measured across the whole surface. \\
%
    \indent As a result, each pixel (covering a quarter degree square on the surface) of the final maps is the result of the weighted average of all the pixels from the individual projections covering the same area. The weight function was defined as a Gaussian-like function of the resolution. This approach returned a larger weight to the best spatial resolution pixels (which are the central one), than for those with lower spatial resolution (further from the center). In addition, thanks to the large number of views used to create each pixel of the map, any remaining artifact would be easily smooth out (values for each map are presented in \textbf{Table \ref{tab-pixmap}})
%
%
%
%%%%%%------ TABLE --- Begin --- Maps per Pixel ------%%%%%%
\begin{table}
  \caption{Number of images per pixel combined to produce final maps, as well as the total surface coverage of each map (on the Ceres surfce).}
  \label{tab-pixmap}
  \centering
  \begin{tabular}{c c c c}
    \hline\hline
    Filter &   Average   &   Max   &  Coverage (\%)\\
    \hline
    J   &   16 img.   &   63 img.  &  81.8\%  \\
    H   &   14 img.   &   54 img.  &  74.2\%  \\
    K   &   19 img.   &   72 img.  &  80.0\%  \\
    \hline
\end{tabular}
\end{table}
%%%%%%------ TABLE ---  End  --- Maps per Pixel ------%%%%%%
%
%
%
%
%
%
%%%%%%------ Leveling the maps for comparison ------%%%%%%
    \paragraph*{Conversion into reflectance :} No absolute calibration was available to calibrate our set of images within each waveband. We therefore used a near infrared disk-integrated spectrum of Ceres [R.Binzel, personal communication] normalized to 1.0 at 0.5 \micron~to calculate the equivalent disk-integrated photometric value for each bands and use it to normalize our maps.
%
%
%
%%%%%%------ FIGURE --- Begin --- J-/H-/K-band Maps ------%%%%%%
\begin{figure*}[!h]
  \centering
  \includegraphics[width=17cm]{JHK-maps}
    \caption{J-, H- and K-band maps of Ceres. Each map covers more or less 80 percent of Ceres surface, with the white area corresponding to the non-mapped surface. The resolution element (that is 36.8 km, 47.4 km and 62.9 km for each band) is placed in the bottom-right corner of each map. The amplitude of the albedo variations are within $\sim$12\% ($\pm$1\% uncertainty) around the mean surface value for each map and the color scale placed on the right side in common for the three filters. These maps match perfectly the UV/Visible HST maps published by \citet{2006-Icarus-182-Li}.}
    \label{fig-jhk-maps}
\end{figure*}
%%%%%%------ FIGURE --- Begin --- J-/H-/K-band Maps ------%%%%%%
%
%
%
%
%%%%%%------ Maps description and informations ------%%%%%%
    \paragraph*{Maps description :} The maps we obtained are shown in \textbf{Fig. \ref{fig-jhk-maps}}. They are the result of the combination of 126, 99 and 135 individual projections in the J-, H- and K-band resp. They are covering roughly 80 percent of Ceres total surface (see \textbf{Tab. \ref{tab-pixmap}}). The gaps in the surface coverage are partly due to a lack of observation around the 330\degr E region, the rest being the result of the limited ROI used to make the maps. The smallest feature visible are the size of the resolution element for  J-, H- and K-band, that is 36.8 km, 47.4 km and 62.9 km resp. (corresponding to 4.4\degr, 5.6\degr and 7.5\degr at the equator). One can easily recognize the main feature seen in our near-infared maps, with the main features displayed in the UV/Visible HST maps published by \citet{2006-Icarus-182-Li} (we used the same reference meridian (0\degr) to help reading). The amplitude of the features are within $\sim$12 $\pm$1\% around the mean surface value for each band. Such low albedo variation across the surface of Ceres was expected from its low amplitude lightcurve. Nevertheless, high-angular resolution imaging of the surface of Ceres reveal a wealth of  albedo marks on a small spatial scale which might be attributed to different collisional history, un-homogeneous space weathering or surface/sub-surface activity.
%
%
%
%
%
%
%
%
  \subsection{Three-points spectra}
%
%
%
%%%%%%------ FIGURE --- Begin --- 3-point spectra ------%%%%%%
%%%--- Vertical Version
% \begin{figure}
% \centering
%   \resizebox{.9\hsize}{!}{\includegraphics{spectra-dark}}
%   \resizebox{.9\hsize}{!}{\includegraphics{spectra-bright}}
%   \caption{Three-point spectra of selected features. Upper panel shows results for \textbf{dark} features and lower panel for \textbf{bright} ones. All the spectra are vertically shifted to help reading and we plotted the Ceres disk-integrated spectrum for reference. The number near the left end of each 3-point spectrum is used to mark the feature position on the map under the spectra. Due to the error bar size, we cannot detect any trend in the slopes.}
%   \label{fig-spectra}
% \end{figure} 
%%%--- Horizontal Version
\begin{figure*}
\centering
  \includegraphics[width=8cm]{spectra-dark}
  \includegraphics[width=8cm]{spectra-bright}
  \caption{Three-point spectra of selected features. Left panel shows results for dark features and right panel for bright ones. All the spectra are vertically shifted to help reading and we plotted the Ceres disk-integrated spectrum [R. Binzel, personal communication] for reference. The number near the left end of each 3-point spectrum is used to localize the feature on the map under the spectra. Due to the error bar size, physical interpretation of broad band variation is not possible. We do not report any trend in the slopes.}
  \label{fig-spectra}
\end{figure*}
%%%%%%------ FIGURE --- End --- 3-point spectra ------%%%%%%
%
%
%
%
%%%%%%------ FIGURE --- Begin --- Ice Dectection------%%%%%%
\begin{figure}
%%%--- Graphics from the EPS and Caption
  \resizebox{.99\hsize}{!}{\includegraphics{ice-detection}}
%%%--- Nom des filtres
  \setlength{\unitlength}{\hsize}
  \begin{pspicture}(0.1,0.01)
    \put(2.3,7.8){\large{J}}
    \put(4.0,7.4){\large{H}}
    \put(6.6,7.1){\large{K}}
  \end{pspicture}

  \caption{Results from the simulation in the cases of 1\% and 4\% frost surface coverage. The upper panel shows the broad band values expected (black) as well as the disk integrated photometry of Ceres for reference (gray). The lower panel shows the ratio between simulated spectra with the disk integrated one. We shifted the results for the different cases to help reading. We see that spectroscopy is of course a much more powerful tool to remotely investigate surface composition of distant bodies.}

  \label{fig-ice-detection}
\end{figure}
%%%%%%------ FIGURE --- End --- Ice Dectection ------%%%%%%
%
%
%
    \indent To attempt investigating further the nature of the major features seen in our 3-color maps, we attempted to report their JHK photometric values against the disk averaged spectrum of Ceres. We selected 17 features (9 bright and 8 dark) and we present their photometric measurements in \textbf{Fig. \ref{fig-spectra}}. The figure shows clearly that no absolute color trend can be determined between dark and bright regions on the surface of Ceres. This lack of diagnostic is mainly due to the large error bars that our photometric determination is suffering (relative uncertainty of about 8\%). If we push further this analysis, it could be possible that the bright features display an excess of intensity in the H-band with respect to the dark ones, but a better photometric accuracy is needed to definitively report on the spectral behavior of these albedo marks. Another limitation hampering the quality of our analysis is due to the poor spectral resolution returned by the broad band filters, and we could expect a much better physical and compositional analysis of the surface albedo features to be possible if one use a combination of adaptive optics and infrared spectroscopy. 

    \indent To illustrate this limitation, we simulated the spectrum and the broad filter values of Ceres if it were partly covered by frost as suggested by \citet{1981-Icarus-48-Lebofsky} (we obtained the water frost spectrum from the ASTER library). As shown by \citet{1989-Icarus-82-Fanale}, water ice is not stable on Ceres surface, so we suppose a fresh excavation from sub-surface layer via an impact crater, covering a given percent of the surface depending on the crater size.\\
%
    \indent In this simple simulation, we supposed that the water frost has the same albedo in H-band as Ceres surface in general, this is reasonable if we suppose a mix with spectral neutral carbonates which have been detected by \citet{2006-Icarus-185-Rivkin}. We realized the simulation in the hypothesis cases of 1\% and 4\% of the surface covered by frost. The upper part of \textbf{Fig. \ref{fig-ice-detection}} shows what we can expect from a broad band analysis and the lower part from spectral analysis. We see that at least 4 percent of the surface need to be covered to allow marginal detection (via J-band deviation) from broad band analysis. But we actually need more than 14 percent to see any K-band deviation, necessary to an unambiguous detection. On the other hand, spectral analysis allows detection down to only one percent of covered surface.

    \indent This simulation shows that we cannot hope water ice remotely detected by broad band analysis. But it confirms the necessity to perform spectroscopic observations. Although disk-integrated spectrum analysis of Ceres in the [1.0, 2.4] \micron~range never report such detection, it was expectable. Indeed, 4\% (1\%) surface coverage for a full hemisphere correspond to a crater radius of $\sim$93 km ($\sim$47 km resp.). To obtain such great surface coverage, it would requiere a recent major impact which would have probably provoced the existence of a family (not detected) or a huge number of small recent craters (which does not seem probable). But water ice, if present, may appears on spatially limited spots on which a few tenth of percent coverage is not unreasonable. So the conduction of integral-field spectroscopy at smal spatial scale should answers to the question of water ice presence. This could be perform from ground telescopes feed by AO like SINFONI/VLT, OSIRIS/Keck II or NIFS/Gemini for example and of course by the DAWN mission with its spatial resolution down to 340 m \citep{2006-AdSpR-38-Russel}.
%
%
%
%
%
%
%
  \subsection{3-D model}
%
    \indent We also used our multicolor map of Ceres to re-project them onto a 3D shape model of the asteroid. Such a model allows us to see Ceres from any sub-observer point. This photometric model can be used to verify the end result of our data processing and analysis by comparing the model with the real data obtained after deconvolution (see \textbf{Fig. \ref{fig-3DvsIM}}). Another use of this model is to predict what Ceres surface would look like at any epochs. This feature will certainly be very useful to prepare future ground-based, or space based observations of Ceres with Dawn.\\
%
%
%
%
%%%%%%------ FIGURE --- Begin --- 3D model ------%%%%%%
% \begin{figure} 
%   \resizebox{\hsize}{!}{\includegraphics{3DviewsK}}
%   \caption{Synthetic views of Ceres. Sub-Observer Point coordinates are (233\degr E, 7\degr N) for the left view and (127\degr E,7\degr N) for the right one. The black areas correspond to the non-mapped surface.}
%   \label{fig-3D-model}
% \end{figure}
%%%%%%------ FIGURE --- End --- 3D model ------%%%%%%
%
%
%
%
%%%%%%------ FIGURE --- Begin --- 3D VERSUS IMAGE------%%%%%%
\begin{figure}
%%%--- Graphics from the EPS and Caption
  \resizebox{\hsize}{!}{\includegraphics{3DvsImage}}
%%%--- Nom des filtres
  \setlength{\unitlength}{\hsize}
  \begin{pspicture}(0.1,0.01)
    \put(1.5,0.7){\large{\textbf{Synthetic}}}
    \put(6.1,0.7){\large{\textcolor{white}{\textbf{Original}}}}
  \end{pspicture}

  \caption{Comparison between a synthetic view (left) and a Ceres deconvolved image (right). The overplotted ellipse correspond to the ROI limit (80\% of projected axis). The features seen outside the ROI on the synthetic view were obtained by combining other images. This kind of comparaison was of great help to check our projection algorithm. The features match between the two views but seem ``smoothed'' in the synthetic one due to the average between many deconvolved images. The only remarkable difference between the synthetic view and the original is situated in the bottom-right area of the ROI and appears dark in the synthetic. This show the importance of combining the data via a weighted average, to only keep the trends and not the unique features among the images.}
  \label{fig-3DvsIM}
\end{figure}
%%%%%%------ FIGURE --- End --- 3D VERSUS IMAGE ------%%%%%%

